Vehicle-Rear: A New Dataset to Explore Feature Fusion for Vehicle Identification Using Convolutional Neural Networks

This work addresses the problem of vehicle identification through non-overlapping cameras. As our main contribution, we introduce a novel dataset for vehicle identification, called Vehicle-Rear, that contains more than three hours of high-resolution videos, with accurate information about the make, model, color and year of nearly 3,000 vehicles, in addition to the position and identification of their license plates. To explore our dataset we design a two-stream CNN that simultaneously uses two of the most distinctive and persistent features available: the vehicle's appearance and its license plate. This is an attempt to tackle a major problem: false alarms caused by vehicles with similar designs or by very close license plate identifiers. In the first network stream, shape similarities are identified by a Siamese CNN that uses a pair of low-resolution vehicle patches recorded by two different cameras. In the second stream, we use a CNN for OCR to extract textual information, confidence scores, and string similarities from a pair of high-resolution license plate patches. Then, features from both streams are merged by a sequence of fully connected layers for decision. In our experiments, we compared the two-stream network against several well-known CNN architectures using single or multiple vehicle features. The architectures, trained models, and dataset are publicly available at https://github.com/icarofua/vehicle-rear.

==> figures/architectures.tex <==
\begin{figure*}
\hspace{-10pt}\input{figures/two_stream_shape_plate}
\hspace{-5pt}\input{figures/three_stream}
\hspace{-10pt}\input{figures/two_stream_shape_ocr}

\caption{Alternative architectures for vehicle re-identification: (a) a two-stream siamese network based on image features extracted from the license plate region and from the vehicle shape; (b) a three-stream network based on image and textual features extracted from the license plate region, and image features extracted from the vehicle shape; and (c) a temporal two-stream network based on image features extract from a sequence of images and textual features extracted from the same sequence.}
\label{fig:architectures}
\end{figure*}

==> figures/junk.tex <==


%We notice that the object appearance in a sequence of consecutive frames often has small image variations --- due to the vehicle motion, scene illumination changes, image noise, compression artifacts, etc --- that usually produce distinct image matching outcomes. Therefore, to evaluate such variations, we used the MOSSE tracker~\cite{} to extract the $n$ first  occurrences of each license plate. See Fig~\ref{}.


%by using region tracking and we consider three scenarios for vehicle matching.

%The first scenario contain all occurrences extracted from each license plate or each rear end of the vehicle. Firstly, we applied the cartesian product between all images from a video of the Camera 1 with the same video in the Camera 2 to obtain the pair of images, with pair get one class equals or different. After, We separated these images into training and testing datasets. We got in the training set 1730117 pair of images formed by 1687150 negative pairs and 42967 positive pairs and in the testing set 1728690 pair of images formed by 1685120 negative pairs and 43570 positive pairs.

%The second scenario is formed by the pairs of the testing set that the license plate had a difference until 4 characters. The third scenario is formed by the pairs of the testing set that the car features are similar, as same brands, same color and the model is 60\% similar.


 where $|tp|$ denotes the number of true matchings between Cameras 1 and 2, $|fp|$ is the number of false matchings, $|fn|$ the number of true matchings missed by the algorithm, and $|tn|$ is the number of true non-matching pairs. For  ranking  purposes,  we  also  consider  the $F$-measure, which  is  the  harmonic  mean  of  precision  and recall 
 
 

REFAZER/REVISAR: As shown in Table~\ref{tb:results}, the Two-Stream Siamese outperforms two distinct One-Stream Siamese Networks: the first one, Siamese-Car, is fed only with the shape of vehicles ($96 \times 96$ pixels); the second, Siamese-Plate, only use patches of license plates ($96 \times 48$ pixels). Note that even when we increased the number of false matchings in the negative testing set, $\lambda=10$, the $F$-measure of the Two-Stream Siamese was similar in both scenarios.  Some inference results are shown in Fig.~\ref{fig:results}.


We also tried different CNN in our Two-Stream Siamese, their performance are reported in Table~\ref{tb:results2}.
Furthermore, as can be seen in Fig.~\ref{fig:results2}, we also evaluated the performance of the proposed Two-Stream Siamese against two One-Stream Siamese versions fed with larger image patches ($224 \times 224$ pixels). Note that we achieved a higher $F$-measure by using two small image patches than a single patch containing both features. Another advantage is the Two-Stream Siamese training time: 1938 seconds per epoch ($N = 10$ and $\lambda = 10$) against 3441 seconds per epoch of the Siamese-Car by using the same Small-VGG and 4937 seconds with ResNet~\cite{resnet}. %Furthermore, the predict time of our Two-Stream Siamese 0.7 ms against 3 ms of the Siamese-Car by using the same Small-VGG and 5 ms with ResNet~\cite{resnet}.

% It is important to highlight that we used the same datasets as Laroca et al.~\cite{laroca2019efficient}, which were proposed by several research groups from different countries, with only 500 more images belonging to our scenario to train the CNN-OCR architecture so that it is robust for various license plate layouts.

* Incluir uma figura de resultados do OCR para diferentes layouts e um pequeno texto a respeito. \RL{ver figura 9, era essa a ideia?!}

% * Atualizar tabela só com os resultados do OCR \RL{Done}

* Na figura 9 colocar exemplos que o OCR falha e o veiculo acerta, que o veiculo falha e o OCR acerta, que os dois acertam e etc! \RL{Essa é com o Icaro}

%As can be seen from Table~\ref{tb:results2} the performance of the Siamese (Two-Stream) using our model is better than the another models as Luoetal, Lenet5, Simple and Small-VGG, in other words, our model extract the best features from car and license plate.




%To compute the SIFT-Plate performance we consider a license plate matching whenever we found at least 12 feature matchings from a given image from Camera 1 with another one in Camera 2. And we consider a car (rear end of the vehicle) matching whenever we found at least 11 feature matchings for the SIFT-Car strategy. 

%As can be seen from Table~\ref{tb:results} the performance of the SIFT-Plate strategy is lower than the SIFT-Car, which means that the rear end of the vehicle has many distinctive features for vehicle identification. However, the average execution time for the feature description and matching of the SIFT-Plate strategy is 0.02 seconds, while the average execution time of the SIFT-Car strategy is 0.35 seconds. In general, this execution time difference is due to the size of the vehicle rear end, which is in average 32 times larger than the license plate as shown in Figure~\ref{falses_sift}. As can be seen the two cases are same in license plates and rear of the end of the vehicle, in other words, SIFT-Plate obtained more than 12 feature matchings and SIFT-Car obtained more than 11 feature matchings.

%\begin{figure}[!ht]lse_sift_plate.png}} 
%  \subfigure[False positive SIFT-Car]{\includegraphics[width=0.49\linewidth]{./figures/false_sift_car.png}}
%  \caption{The false positives in SIFT-Plate (axt-8589 vs axc-9549) and in SIFT-Car (aus-1730 vs aus-1729). }  
%  \label{falses_sift}
%\end{figure}

%\begin{figure}[!ht]
%  \centering
%  \includegraphics[width=1.0\linewidth]{./figures/falses_siamese.png}
%  \caption{The false positives in Siamese-Plate (azg-3589 vs axt-8589) and in Siamese-Car (aus-1729 vs aus-1730) where Siamese-Plate missed with 65,6\% and Siamese-Car with 99,82\%. The false positives in Siamese-Concat (azg-3589 vs axt-8589) and (aus-1729 vs aus-1730) where Siamese-Concat missed with 99,9\% and with 99,82\%. The false positives in Siamese-Pair (azg-3589 vs axt-8589) and (aus-1729 vs auf-2796) where Siamese-Pair missed with 66,5\% and with 99,62\%. The false positives in Siamese-Voting (aus-1729 vs aus-1730) and (ayr-5217 vs ayb-5619). } 
%  \label{falses_siamese1}
%\end{figure}

%\begin{figure}[!ht]
%  \centering
%  \includegraphics[width=1.0\linewidth]{./figures/falses_siamese2.png}
%  \caption{The false positives in Siamese-Plate (azg-3589 (B) vs axt-8589 (C)) and in Siamese-Car (aus-1729 (E) vs aus-1730 (A)) where Siamese-Plate missed with 65,6\% and Siamese-Car with 99,82\%. The false positives in Siamese-Concat (azg-3589 (B) vs axt-8589 (C)) and (aus-1729 (D) vs aus-1730 (A)) where Siamese-Concat missed with 99,9\% and with 99,82\%. The false positives in Siamese-Pair (azg-3589 (B) vs axt-8589 (C)) and (aus-1729 (D) vs auf-2796 (E)) where Siamese-Pair missed with 66,5\% and with 99,62\%. The false positives in Siamese-Voting (aus-1729 (D) vs aus-1730 (A)) and (ayr-5217(F) vs ayb-5619 (G)). } 
%  \label{falses_siamese2}
%\end{figure}

%As shown in Figure~\ref{falses_siamese1}, the Siamese-Plate with TFS obtained the performance (76.0\% vs 74.1\%) better than SIFT-Plate and the average execution time for this method is 0.02 seconds. The Siamese-Car with TFS and SIFT-Car obtained the same performance 86.0\%, the average execution time for this method is 0.02 seconds. But, the Siamese-Plate didn't have the same false positive than SIFT-Plate and we used a image smaller (56 x 64) than SIFT-Car and obtained the same performance with a average execution time two times smaller than SIFT-Car. 

%The Siamese-Concat with LENET5 is the same performance than Siamese-Car, in other words, the rear of the end of vehicle region is prevalent in the Siamese-Concat. The average execution time for this method is 0.02 seconds. But, this model obtained the same false positives of the Siamese-Plate and Siamese-Car and the miss probability of the Siamese-Plate´s false positive is 34\% greater than Siamese-Plate. 

%The Siamese-Pair with VGG\_1024 obtained the second best performance than all previous 87.0\%, the Siamese-Pair extracted distinct features from the best regions between the two images license plate and rear end of the vehicle. The average execution time for this method is 0.04 seconds. This model can filter the positive false (aus-1729 vs aus-1730) but obtained another same false positive (aus-1729 vs auf-2796), furthermore the miss probability of the Siamese-Plate´s false positive is 0,9\% greater than Siamese-Plate, in other words, it is 33,4\% smaller than Siamese-Concat. 

%Finally, the Siamese-Voting obtained the better performance than all methods 90.4\%, the average execution time for this method is 0.11 seconds. This model filtered all false positives of the axt-8589, but obtained the Siamese-Car´s false positive (aus-1729 vs aus-1730) because this false positive is showed in Siamese-Car and Siamese-Plate models obtained two votings versus one voting from Siamese-Pair. Furthermore, we showed the results in the others two scenarios in the Table~\ref{tb:results2}, the same Siamese-Votings' false positives are found in the two scenarios, because these are falses positives with similar cars and similar license plates.

%\begin{table}[ht]
%\renewcommand{\arraystretch}{1.3}
%\setlength{\tabcolsep}{7pt}
%\def\de{\small}
%\centering
%\caption{Matching scores for the method proposed in the second and third scenarios.}
%\label{tb:results2}
%\begin{tabular}{|l||c|c|c|c|} \hline
%\de Scenario  & \de   $P$   &\de   $R$   &\de   $F$   &\de   $A$ \\ \hline
%\de Second &\de   91.0\%   &\de   91.2\%   &\de   91.0\%   &\de    99.2\%  \\ \hline  
%\de Third &\de   96.3\%   &\de   91.2\%   &\de   94.0\%   &\de    90.0\%  \\ \hline  
%\end{tabular}
%\end{table}

%As can be seen from Figure~\ref{fig:results2} the Siamese Two-Stream (Small-VGG) obtained the performance (92.6\% vs 88.1\% vs 81.2\%) better than Siamese-Car (Small-VGG) and Siamese-Car (Resnet50), respectively and more efficient (0.7ms vs 3ms vs 5ms) than Siamese-Car (Small-VGG) and Siamese-Car (Resnet50),respectively.

%As can be seen from Figure~\ref{fig:results} in three scenarios the Siamese (Two-Stream) was better than Siamese-Car and Siamese-Plate but in the first scenario the result was wrong in all three methods because the sun in the car makes it brighter in the first pair from Camera 1 than the second pair from Camera 2. The second scenario is a problem for car because the two cars are similar but license plate is different. The third scenario shows the same car and license plate but because the viewpoint the Siamese-Plate wrong the result. Finally, in the fourth scenario all the methods are right because the two pairs are very different between them.

CNN = Resnet8 ($128\times128$ px)  & 86.86\% & 87.96\% & 87.04\%\\

